JarKA: Modeling Attribute Interactions for Cross-lingual Knowledge Alignment

Abstract. Cross-lingual knowledge alignment is the cornerstone in building a comprehensive knowledge graph (KG), which can benefit various knowledge-driven applications. As the structures of KGs are usually sparse, attributes of entities may play an important role in aligning the entities. However, the heterogeneity of the attributes across KGs prevents from accurately embedding and comparing entities. To deal with the issue, we propose to model the interactions between attributes, instead of globally embedding an entity with all the attributes. We further propose a joint framework to merge the alignments inferred from the attributes and the structures. Experimental results show that the proposed model outperforms the state-of-art baselines by up to 38.48% HitRatio@1. The results also demonstrate that our model can infer the alignments between attributes, relationships and values, in addition to entities.

==> reference.tex <==
\begin{thebibliography}{8}
\bibitem{ref_article1}
Author, F.: Article title. Journal \textbf{2}(5), 99--110 (2016)

\bibitem{ref_lncs1}
Author, F., Author, S.: Title of a proceedings paper. In: Editor,
F., Editor, S. (eds.) CONFERENCE 2016, LNCS, vol. 9999, pp. 1--13.
Springer, Heidelberg (2016). \doi{10.10007/1234567890}

\bibitem{ref_book1}
Author, F., Author, S., Author, T.: Book title. 2nd edn. Publisher,
Location (1999)

\bibitem{ref_proc1}
Author, A.-B.: Contribution title. In: 9th International Proceedings
on Proceedings, pp. 1--2. Publisher, Location (2010)

\bibitem{ref_url1}
LNCS Homepage, \url{http://www.springer.com/lncs}. Last accessed 4
Oct 2017

@article{ahlander2002einstein,
	title={Einstein summation for multidimensional arrays},
	author={Ahlander, Krister},
	journal={Computers \& Mathematics With Applications},
	volume={44},
	pages={1007--1017},
	year={2002}}

@inproceedings{papineni2002bleu,
	title={BLEU: a method for automatic evaluation of machine translation},
	author={Papineni, Kishore and Roukos, Salim and Ward, Todd and Zhu, Wei-Jing},
	booktitle={Proceedings of the 40th annual meeting on association for computational linguistics},
	pages={311--318},
	year={2002},
	organization={Association for Computational Linguistics}
}

@inproceedings{bahdanau2015neural,
	title={Neural Machine Translation by Jointly Learning to Align and Translate},
	author={Bahdanau, Dzmitry and Cho, Kyunghyun and Bengio, Yoshua},
	booktitle={Proceedings of the 6th International Conference on Learning Representations},
	year={2015}
}


@inproceedings{bordes2013translating,
	title={Translating embeddings for modeling multi-relational data},
	author={Bordes, Antoine and Usunier, Nicolas and Garcia-Duran, Alberto and Weston, Jason and Yakhnenko, Oksana},
	booktitle={Proceedings of the 27th Conference on Neural Information Processing Systems},
	pages={2787--2795},
	year={2013}
}


@inproceedings{cao2019multi,
	title={Multi-Channel Graph Neural Network for Entity Alignment},
	author={Cao, Yixin and Liu, Zhiyuan and Li, Chengjiang and Li, Juanzi and Chua, Tat-Seng},
	booktitle={Proceedings of the 57th Conference of the Association for Computational Linguistics},
	pages={1452--1461},
	year={2019}
}
@inproceedings{chen2017multilingual,
	title={Multilingual Knowledge Graph Embeddings for Cross-lingual Knowledge Alignment},
	author={Chen, Muhao and Tian, Yingtao and Yang, Mohan and Zaniolo, Carlo},
	booktitle = {Proceedings of the 26th International Joint Conference on Artificial Intelligence},
	pages={1511--1517},
	year={2017}}

@inproceedings{chen2018co-training,
	title={Co-training Embeddings of Knowledge Graphs and Entity Descriptions for Cross-lingual Entity Alignment},
	author={Chen, Muhao and Tian, Yingtao and Chang, Kaiwei and Skiena, Steven and Zaniolo, Carlo},
	booktitle={Proceedings of the 27th International Joint Conference on Artificial Intelligence},
	pages={3998--4004},
	year={2018}
}

@inproceedings{conneau2017word,
	title={Word translation without parallel data},
	author={Conneau, Alexis and Lample, Guillaume and Ranzato, Marc'Aurelio and Denoyer, Ludovic and J{\'e}gou, Herv{\'e}},
	booktitle={Proceedings of the 6th International Conference on Learning Representation},
	year={2018}
}

@inproceedings{hao2016joint,
	title={A joint embedding method for entity alignment of knowledge bases},
	author={Hao, Yanchao and Zhang, Yuanzhe and He, Shizhu and Liu, Kang and Zhao, Jun},
	booktitle={China Conference on Knowledge Graph and Semantic Computing},
	pages={3--14},
	year={2016},
}

@inproceedings{kipf:17,
	title={Semi-supervised classification with graph convolutional networks},
	author={Kipf, Thomas N and Welling, Max},
	booktitle={Proceedings of the 8th International Conference on Learning Representations},
	year={2017}
}


@inproceedings{wang2012cross,
	title={Cross-lingual knowledge linking across wiki knowledge bases},
	author={Wang, Zhichun and Li, Juanzi and Wang, Zhigang and Tang, Jie},
	booktitle={Proceedings of the 21st International Conference on World Wide Web},
	pages={459--468},
	year={2012},
}


@inproceedings{lacoste2013sigma,
	title={Sigma: Simple greedy matching for aligning large knowledge bases},
	author={Lacoste-Julien, Simon and Palla, Konstantina and Davies, Alex and Kasneci, Gjergji and Graepel, Thore and Ghahramani, Zoubin},
	booktitle={Proceedings of the 19th ACM SIGKDD International Conference on Knowledge Discovery and Data Mining},
	pages={572--580},
	year={2013},
}
booktitle={SIGKDD'13},

@inproceedings{lin2015learning,
	title={Learning entity and relation embeddings for knowledge graph completion},
	author={Lin, Yankai and Liu, Zhiyuan and Sun, Maosong and Liu, Yang and Zhu, Xuan},
	booktitle={Proceedings of the 29th AAAI Conference on Artificial Intelligence},
	pages={2181--2187},
	year={2015}
}

@inproceedings{liu:16IJCAI,
	title={Aligning Users across Social Networks Using Network Embedding.},
	author={Liu, Li and Cheung, William K and Li, Xin and Liao, Lejian},
	booktitle={Proceedings of the 25th International Joint Conference on Artificial Intelligence},
	pages={1774--1780},
	year={2016},
}
booktitle={IJCAI'16},

@inproceedings{liu:17IJCAI,
	author    = {Liu, Lin and LI, Xin and Cheung,  William K. and Xu,  Chengcheng},
	title     = {A Structural Representation Learning for Multi-relational Networks},
	booktitle = {Proceedings of the 26th International Joint Conference on
		Artificial Intelligence},
	pages     = {4047--4053},
	year      = {2017},
}

@inproceedings{Li:18IJCAI,
	author    = {Li, Shengnan and Li, Xin and Ye, Rui and Wang, Mingzhong and Su, Haiping and Ou, Yingzi},
	title     = {Non-translational Alignment for Multi-relational Networks},
	booktitle = {Proceedings of the 27th International Joint Conference on
		Artificial Intelligence},
	year      = {2018},
}




@inproceedings{man:16IJCAI,
	title={Predict Anchor Links across Social Networks via an Embedding Approach.},
	author={Man, Tong and Shen, Huawei and Liu, Shenghua and Jin, Xiaolong and Cheng, Xueqi},
	booktitle={Proceedings of the 25th International Joint Conference on Artificial Intelligence},
	pages={1823--1829},
	year={2016},
}
booktitle={IJCAI'16},


@article{nguyen2011multilingual,
	title={Multilingual schema matching for Wikipedia infoboxes},
	author={Nguyen, Thanh and Moreira, Viviane and Nguyen, Huong and Nguyen, Hoa and Freire, Juliana},
	journal={Proceedings of the VLDB Endowment},
	volume={5},
	number={2},
	pages={133--144},
	year={2011},
}




@inproceedings{niu2012effective,
	title={An effective rule miner for instance matching in a web of data},
	author={Niu, Xing and Rong, Shu and Wang, Haofen and Yu, Yong},
	booktitle={Proceedings of the 21st ACM International Conference on Information and Knowledge Management},
	pages={1085--1094},
	year={2012},
}


@inproceedings{oh2008enriching,
	title={Enriching multilingual language resources by discovering missing cross-language links in wikipedia},
	author={Oh, Jong-Hoon and Kawahara, Daisuke and Uchimoto, Kiyotaka and Kazama, Jun'ichi and Torisawa, Kentaro},
	booktitle={2008 IEEE/WIC/ACM International Conference on Web Intelligence and Intelligent Agent Technology},
	volume={1},
	pages={322--328},
	year={2008},
}


@inproceedings{pershina2015holistic,
	title={Holistic entity matching across knowledge graphs},
	author={Pershina, Maria and Yakout, Mohamed and Chakrabarti, Kaushik},
	booktitle={2015 IEEE International Conference on Big Data},
	pages={1585--1590},
	year={2015},
}


@article{rinser2013cross,
	title={Cross-lingual entity matching and infobox alignment in Wikipedia},
	author={Rinser, Daniel and Lange, Dustin and Naumann, Felix},
	journal={Information Systems},
	volume={38},
	number={6},
	pages={887--907},
	year={2013},
}

@inproceedings{sorg2008enriching,
	title={Enriching the crosslingual link structure of wikipedia-a classification-based approach},
	author={Sorg, Philipp and Cimiano, Philipp},
	booktitle={Proceedings of the AAAI 2008 Workshop on Wikipedia and Artifical Intelligence},
	year={2008}
}


@inproceedings{sun2017crosslingual,
	title={Cross-Lingual Entity Alignment via Joint Attribute-Preserving Embedding},
	author={Sun, Zequn and Hu, Wei and Li, Chengkai},
	booktitle={Proceedings of the 16th International Semantic Web Conference},
	pages={628--644},
	year={2017}}

@article{suchanek2011paris,
	title={Paris: Probabilistic alignment of relations, instances, and schema},
	author={Suchanek, Fabian M and Abiteboul, Serge and Senellart, Pierre},
	journal={Proceedings of the VLDB Endowment},
	volume={5},
	number={3},
	pages={157--168},
	year={2011},
}


@inproceedings{sun2018bootstrapping,
	title={Bootstrapping Entity Alignment with Knowledge Graph Embedding},
	author={Sun, Zequn and Hu, Wei and Zhang, Qingheng and Qu, Yuzhong},
	booktitle={Proceedings of the 27th International Joint Conference on Artificial Intelligence},
	pages={4396--4402},
	year={2018}}

@inproceedings{Trsedya2019,
	title={Entity Alignment between Knowledge Graphs Using Attribute Embeddings},
	author={Bayu Distiawan Trsedya and Jianzhong Qi and Rui Zhang},
	booktitle={Proceedings of the 33rd AAAI Conference on Artificial Intelligence},
	year={2019}}

@inproceedings{wang2013boosting,
	title={Boosting cross-lingual knowledge linking via concept annotation},
	author={Wang, Zhichun and Li, Juanzi and Tang, Jie},
	booktitle={Proceedings of the 23rd International Joint Conference on Artificial Intelligence},
	pages={2733--2739},
	year={2013}
}


@inproceedings{wang2014knowledge,
	title={Knowledge graph embedding by translating on hyperplanes},
	author={Wang, Zhen and Zhang, Jianwen and Feng, Jianlin and Chen, Zheng},
	booktitle={Proceedings of the 28th AAAI Conference on Artificial Intelligence},
	pages={1112--1119},
	year={2014}
}

@inproceedings{wang2018cross,
	title={Cross-lingual Knowledge Graph Alignment via Graph Convolutional Networks},
	author={Wang, Zhichun and Lv, Qingsong and Lan, Xiaohan and Zhang, Yu},
	booktitle={Proceedings of the 2018 Conference on Empirical Methods in Natural Language Processing},
	pages={349--357},
	year={2018}
}

@article{wu2016google,
	title={Google's neural machine translation system: Bridging the gap between human and machine translation},
	author={Wu, Yonghui and Schuster, Mike and Chen, Zhifeng and Le, Quoc V and Norouzi, Mohammad and Macherey, Wolfgang and Krikun, Maxim and Cao, Yuan and Gao, Qin and Macherey, Klaus and others},
	journal={arXiv preprint arXiv:1609.08144},
	year={2016}
}


@inproceedings{xu2019cross,
	title={Cross-lingual Knowledge Graph Alignment via Graph Matching Neural Network},
	author={Xu, Kun and Wang, Liwei and Yu, Mo and Feng, Yansong and Song, Yan and Wang, Zhiguo and Yu, Dong},
	booktitle={Proceedings of the 57th Conference of the Association for Computational Linguistics},
	pages={1452--1461},
	year={2019}
}



@inproceedings{zhang2018mego2vec,
	title={MEgo2Vec: Embedding Matched Ego Networks for User Alignment Across Social Networks},
	author={Zhang, Jing and Chen, Bo and Wang, Xianming and Chen, Hong and Li, Cuiping and Jin, Fengmei and Song, Guojie and Zhang, Yutao},
	booktitle={Proceedings of the 27th ACM International Conference on Information and Knowledge Management},
	pages={327--336},
	year={2018},
}

@inproceedings{zhang2019multi,
	title={Multi-view Knowledge Graph Embedding for Entity Alignment},
	author={Zhang, Qingheng and Sun, Zequn and Hu, Wei and Chen, Muhao and Guo, Lingbing and Qu, Yuzhong},
	booktitle={Proceedings of the 33th AAAI Conference on Artificial Intelligence},
	year={2019}
}



@inproceedings{zhong2018colink,
	title={CoLink: An Unsupervised Framework for User Identity Linkage},
	author={Zhong, Zexuan and Cao, Yong and Guo, Mu and Nie, Zaiqing},
	booktitle={Proceedings of the 32nd AAAI Conference on Artificial Intelligence},
	year={2018}
}

@inproceedings{zhu2017iterative,
	title={Iterative Entity Alignment via Joint Knowledge Embeddings},
	author={Zhu, Hao and Xie, Ruobing and Liu, Zhiyuan and Sun, Maosong},
	booktitle = {Proceedings of the 26th International Joint Conference on Artificial Intelligence},
	pages={4258--4264},
	year={2017}}







\end{thebibliography}
